Prescribing the curvature to Killing Graphs

In this work we prove the existence and uniqueness of Killing graphs with prescribed mean curvature considering functions which are not necessarily constant along the flow lines of the Killing vector field.

==> 00README.XXX.tex <==
nohypertex
